Subpixel Mapping and Test Beam Studies with a HV2FEI4v2 CMOS-Sensor-Hybrid Module for the ATLAS Inner Detector Upgrade

The upgrade to the High Luminosity Large Hadron Collider will pose unprecedented challenges to the tracking systems of all experiments. Recent advancement of active pixel detectors designed in CMOS processes provide attractive alternatives to the well-established hybrid design using passive sensors. This article presents studies with a high-voltage CMOS active pixel sensor designed for the ATLAS tracker upgrade. The sensor is glued to the read-out chip of the Insertable B-Layer. The device under test is structured in smaller pixels than those of the attached read-out chip with information on the hit CMOS pixel encoded in the output signal (subpixel encoding). Test beam measurements mapping recorded hits in the read-out chip to CMOS pixels, thus validating the subpixel encoding, are described.

==> sections/usbpix.tex <==
\subsection{Read-out System}\label{sec:usbpix}

Data acquisition and calibration of both the HV2FEI4v2 and the FE-I4 of the CCPD hybrid under study were
carried out with the USBpix system~\cite{Backhaus_USBpix}. Operation of FE-I4 chips (without CMOS sensors) 
with USBpix was fully implemented in the course of module tests for the Insertable B-layer (IBL)~\cite{IBL}.
Existing software provides full integration with the EUDET/AIDA telescope~\cite{EUDET}
which allows test beam measurements, see section~\ref{sec:tbsetup}. 

While communication between USBpix and FE-I4 relies on the programmable didital electronics
of the USBpix main board (Multi-IO), a General Purpose Adapter Card (GPAC) connected to the Multi-IO board
provides additional DC and slow input signals needed to control the HV2FEI4v2. Both
boards are steered by a C++ software package that permits simultaneous control and read-out
of HV2FEI4v2 and FE-I4 as would be required during ATLAS data taking and calibration~\cite{Rieger_USBPix}.

Test and calibration of the HV2FEI4v2 is performed using an internal injection mechanism:
a well-defined charge is injected directly into the
analogue part of all pixels of the HV2FEI4v2 at the same time via the GPAC injection
circuit. The generated signal is then read out by the FE-I4. With a measurement injecting
a charge well above the expected HV2FEI4v2 discriminator threshold, the capacitive coupling of HV2FEI4v2 
to FE-I4 is validated (\textit{Analog Test}). A similar measurement records and possibly adjusts the \ToT measured 
by the FE-I4. A \textit{Threshold Scan} is based on injections with automatically varying the 
injection voltage from the GPAC during the scan. The injection is repeated several times and
the number of hits per injection voltage as measured by the FE-I4 is recorded. During the scan, the injection
voltage is varied from 0~V to 1.5~V in 61 steps. The resulting number of hits as function of the injection voltage
is fitted with an error function. The fit determines the injection voltage at the comparator 
threshold as the voltage at 50\% of the occupancy while the fit parameter describing the spread of the turn-on behaviour
corresponds to the equivalent noise of the HV2FEI4v2 analogue cell.

